Large Language Models Meet Harry Potter: A Bilingual Dataset for Aligning Dialogue Agents with Characters

In recent years, Dialogue-style Large Language Models (LLMs) such as ChatGPT and GPT4 have demonstrated immense potential in constructing open-domain dialogue agents. However, aligning these agents with specific characters or individuals remains a considerable challenge due to the complexities of character representation and the lack of comprehensive annotations. In this paper, we introduce the Harry Potter Dialogue (HPD) dataset, designed to advance the study of dialogue agents and character alignment. The dataset encompasses all dialogue sessions (in both English and Chinese) from the Harry Potter series and is annotated with vital background information, including dialogue scenes, speakers, character relationships, and attributes. These extensive annotations may empower LLMs to unlock character-driven dialogue capabilities. Furthermore, it can serve as a universal benchmark for evaluating how well can a LLM aligning with a specific character. We benchmark LLMs on HPD using both fine-tuning and in-context learning settings. Evaluation results reveal that although there is substantial room for improvement in generating high-quality, character-aligned responses, the proposed dataset is valuable in guiding models toward responses that better align with the character of Harry Potter.

==> tables/case_study.tex <==
\begin{table*}[t]
\vspace{-20pt}
\begin{center}
\footnotesize
\begin{tabular}{ll}
\toprule
\multicolumn{1}{c}{\bf Case 1}  &\multicolumn{1}{c}{\bf Case 2}
\\ \midrule
\begin{minipage}[t]{0.45\textwidth}%
\textbf{Scene}
\\
“And now, Harry, on a closely related subject . . . I gather that you have been taking the Daily Prophet over the last two weeks?”
“Yes,” said Harry, and his heart beat a little faster\dots “— to worry or frighten them?” said Dumbledore, surveying Harry over the top of his half-moon spectacles. “Or perhaps, to confess that you yourself are worried and frightened? You need your friends, Harry. As you so rightly said, Sirius would not have wanted you to shut yourself away.”
\end{minipage}
&
\begin{minipage}[t]{0.45\textwidth}%
\textbf{Scene}
\\
After lunch they went to the reptile house. It was cool and dark in there, with lit windows all along the walls. Behind the glass, all sorts of lizards and snakes were crawling and slithering over bits of wood and stone\dots Dudley was telling them how it had nearly bitten off his leg, while Piers was swearing it had tried to squeeze him to death. But worst of all, for Harry at least, was Piers calming dBelongings enough to say, “Harry was talking to it, weren’t you, Harry?”
\end{minipage}
\\ \\
\begin{minipage}[t]{0.45\textwidth}%
\textbf{Timeline} \\
Book 6-Chapter 4 \\
\textbf{Speakers} \\
Harry and Dumbledore

% Q$_{1}$: Did Cotton live alone? \\
% A$_{1}$: no  \\
% R$_{1}$: Cotton wasn't alone.

\end{minipage}
&
\begin{minipage}[t]{0.45\textwidth}%
\textbf{Timeline} \\
Book 1-Chapter 2 \\
\textbf{Speakers} \\
Harry, Snake, Piers and Dudley
\end{minipage}
\\ \\
\begin{minipage}[t]{0.45\textwidth}%
\textbf{Harry Attributes} \\
Gender: Male \\
Age: 16 \\
Talent: Quidditch, Parseltongue \\
...
\\
Affiliation: Hogwarts \\
Lineage: Pure Blood Wizard \\
Belongings: Holly Phoenix Feather Wand, Owl, Invisibility Cloak, Pocket Looking Glass, Firebolt-Broom, Marauder's Map
\end{minipage}
&
\begin{minipage}[t]{0.45\textwidth}%
\textbf{Harry Attributes} \\
Gender: Male \\
Age: 11 \\
Talent: Parseltongue \\
...
\\
Affiliation: None \\
Lineage: None \\
Belongings: None
\end{minipage}
\\ \\
\begin{minipage}[t]{0.45\textwidth}%
\textbf{Relations} \\
Harry's affection for Dumbledore : 6 \\
Harry's familiarity  with Dumbledore : 6 \\
Harry's affection for Sirius : 8 \\
Harry's familiarity  with Sirius : 6 \\
\textbf{Family} \\
Parents: James Potter and Lily Potter \\
Godfather: Sirius \\
...
\end{minipage}
&
\begin{minipage}[t]{0.45\textwidth}%
\textbf{Relations} \\
Harry's affection for Dudley : -4 \\
Harry's familiarity  with Dudley : 6 \\
Harry's affection for Piers : -3 \\
Harry's familiarity  with Piers : 2 \\
\textbf{Family} \\
Parents: James Potter and Lily Potter \\
Relatives: Dudley, Aunt Petunia and Uncle Vernon \\
...
\end{minipage}
\\\\
\begin{minipage}[t]{0.45\textwidth}%
\textbf{Dialogue} \\
Dumbledore: And now, Harry, on a closely related subject . . . I gather that you have been taking the Daily Prophet over the last two weeks? \\
Harry: Yes \\
...\\
Dumbledore: I think they ought to know. You do them a disservice by not confiding something this important to them. \\
Harry: I didn’t want — \\
Dumbledore: Or perhaps, to confess that you yourself are worried and frightened? You need your friends, Harry. As you so rightly said, Sirius would not have wanted you to shut yourself away.
\\
\\
\textbf{Generated Responses} \\
GPT: I do not need friends.\\
EVA: He wants to, he wants too much.  \\
Ori-BOB:  I think they are meaningless...\\
Per-BOB: It is not your business, because it's my own choice. \\
\textbf{Expected Response}: Yes, Sirius really doesn't want that, maybe I should talk to them.

\end{minipage}
&
\begin{minipage}[t]{0.45\textwidth}%
\textbf{Dialogue} \\
Dudley: Make it move. Do it again...This is boring. \\
Snake: I get that all the time. \\
Harry: I know, it mush be really annoying. Where do you come from, anyway? \\
...\\
Pears: DUDLEY! MR. DURSLEY! COME AND LOOK AT THIS SNAKE! YOU WON’T BELIEVE WHAT IT’S DOING! \\
... \\
Pears: Harry was talking to it, weren't you?
\\
\\
\\
\\
\\
\textbf{Generated Responses} \\
GPT: I do not know... I want to go to Hogwarts.\\
EVA: Sorry, Professor Snape, this is an accident.  \\
Ori-BOB: I think so, Hagrid.  \\
Per-BOB: Let us go to see  Hagrid with my owl.\\
\textbf{Expected Response}: I don't know, you stop talking nonsense, please stop targeting me.
\end{minipage}
\\ \bottomrule
\end{tabular}
\end{center}
\vspace{-10pt}
\caption{Data examples of our dataset and generated responses by baselines (1).}
\vspace{-10pt}
\label{table:case_study}
\end{table*}

==> tables/human_evaluation.tex <==
\begin{table}[t]
    \begin{center}
    \centering
    \small
    % \resizebox{0.8\columnwidth}{!}%
    \begin{tabular}{lcccc}
    \toprule
        \textbf{Model} & \textbf{Flue.}& \textbf{Relv.Sce.} & \textbf{Relv.Att.} & \textbf{Relv.Re.} \\
    \midrule
      GPT-2  & 3.34  &1.68   & 1.9 & 1.5\\
      Dialog-GPT   & \textbf{4.27}&\textbf{2.38}  & \textbf{2.5}& 2.04 \\
      Ori-BOB &4.01  & 1.93 &  1.78&1.9 \\
      Per-BOB &4.2  & 2.01 &  2.16&\textbf{2.15} \\
       

    \bottomrule
    \end{tabular}
    \end{center}
    \caption{
        Human evaluation results of three generation models on the testset of HPD.
    }
    % \vspace{-10pt}
    
    \label{tab:human_evaluation}
\end{table}

==> tables/mapping.tex <==
\begin{table}[t]
    \begin{center}
    \centering
    \small
    % \resizebox{0.8\columnwidth}{!}%
    \begin{tabular}{lcc}
    \toprule
    Score& Relation Mapping  \\
    \midrule
% \multicolumn{3}{c}{\it{per dialogue}}\\
\midrule
    {10} &\multirow{1}{*}{She knows him like the back of her hand}  \\
     {9}&\multirow{1}{*}{9}&\multirow{1}{*}{8}  \\
{Minimum Speakers}&\multirow{1}{*}{2}&\multirow{1}{*}{2}  \\
\midrule
\multicolumn{3}{c}{\it{per sentence}}\\
\midrule
     {Average Length }&\multirow{1}{*}{32.9}&\multirow{1}{*}{28.3}  \\
     
 {Maximum Length}&\multirow{1}{*}{77}&\multirow{1}{*}{31}  \\
      
    {Minimum Length }&\multirow{1}{*}{3}&\multirow{1}{*}{7}  \\
      \midrule
      
{Total Dialogues}&\multirow{1}{*}{1042}&\multirow{1}{*}{178}  \\
        

    
    %  \multicolumn{7}{c}{\it{Train}}\\
     
%      \midrule
%       13.8 & 32.9&77  & 3&20&2&1042 \\
%      \midrule
%         \multicolumn{7}{c}{\it{Test}}\\
%                   \midrule
% 8.6 & 28.3&31  & 7&8&2&178 \\
    \bottomrule
    \end{tabular}
    \end{center}
    \caption{
        Data statics of collected dialogues.
    }
    \label{tab:dialogues}
\end{table}

==> tables/scene_statics.tex <==
\begin{table}[t]
    \begin{center}
    \centering
    \small
    % \resizebox{0.8\columnwidth}{!}%
    \begin{tabular}{lccc}
    \toprule
        \textbf{Book} & \textbf{With Dialogues}& \textbf{Descriptive} & \textbf{Total} \\
    \midrule
      Book-1 & 152&21  & 173 \\
      Book-2    &    320    & 88 & 408 \\
        Book-3       &173   & 11 &  184 \\
         Book-4    &    292    & 8 & 300 \\
        Book-5      &314   & 15 &  329 \\
         Book-6   &    249    & 6 & 255 \\
        Book-7       &291   & 16 &  307 \\
                  \midrule
All & 1791&165&1956  \\
    \bottomrule
    \end{tabular}
    \end{center}
    \caption{
        Data statics of collected scenes.
    }
    \label{tab:scenes}
\end{table}

==> tables/short_case.tex <==
% \begin{table*}[t]
% \vspace{-20pt}
% \begin{center}
% \footnotesize
% \begin{tabular}{ll}
% \toprule
% \multicolumn{1}{c}{\bf Case 1}  &\multicolumn{1}{c}{\bf Case 2}
% \\ \midrule
% \begin{minipage}[t]{0.45\textwidth}%
% \textbf{Scene}
% \\
% “And now, Harry, on a closely related subject . . . I gather that you have been taking the Daily Prophet over the last two weeks?”
% “Yes,” said Harry . . .  As you so rightly said, Sirius would not have wanted you to shut yourself away.”
% \end{minipage}
% &
% \begin{minipage}[t]{0.45\textwidth}%
% \textbf{Scene}
% \\
% After lunch they went to the reptile house. . . But worst of all, for Harry at least, was Piers calming dBelongings enough to say, “Harry was talking to it, weren’t you, Harry?”
% \end{minipage}
% \\ \\
% \begin{minipage}[t]{0.45\textwidth}%
% \textbf{Timeline} \\
% Book 6-Chapter 4 \\
% \textbf{Speakers} \\
% Harry and Dumbledore

% % Q$_{1}$: Did Cotton live alone? \\
% % A$_{1}$: no  \\
% % R$_{1}$: Cotton wasn't alone.

% \end{minipage}
% &
% \begin{minipage}[t]{0.45\textwidth}%
% \textbf{Timeline} \\
% Book 1-Chapter 2 \\
% \textbf{Speakers} \\
% Harry, Snake, Piers and Dudley
% \end{minipage}
% \\ \\
% \begin{minipage}[t]{0.45\textwidth}%
% \textbf{Harry Attributes} \\
% Gender: Male \\
% Age: 16 \\
% Talent: Quidditch, Parseltongue \\
% ...
% \\
% Affiliation: Hogwarts \\
% % Lineage: Pure Blood Wizard \\
% Belongings: Holly Phoenix Feather Wand, ... Firebolt-Broom, Marauder's Map
% \end{minipage}
% &
% \begin{minipage}[t]{0.45\textwidth}%
% \textbf{Harry Attributes} \\
% Gender: Male \\
% Age: 11 \\
% Talent: Parseltongue \\
% ...
% \\
% Affiliation: None \\
% % Lineage: None \\
% Belongings: None
% \end{minipage}
% \\ \\
% \begin{minipage}[t]{0.45\textwidth}%
% \textbf{Relations} \\
% Harry's affection for Dumbledore : 6 \\
% Harry's familiarity  with Dumbledore : 6 \\
% Harry's affection for Sirius : 8 \\
% Harry's familiarity  with Sirius : 6 \\
% % \textbf{Family} \\
% % Parents: James Potter and Lily Potter \\
% % Godfather: Sirius \\
% ...
% \end{minipage}
% &
% \begin{minipage}[t]{0.45\textwidth}%
% \textbf{Relations} \\
% Harry's affection for Dudley : -4 \\
% Harry's familiarity  with Dumbledore : 6 \\
% Harry's affection for Dumbledore : -3 \\
% Harry's familiarity  with Dumbledore : 2 \\
% % \textbf{Family} \\
% % Parents: James Potter and Lily Potter \\
% % Relatives: Dudley, Aunt Petunia and Uncle Vernon \\
% ...
% \end{minipage}
% \\\\
% \begin{minipage}[t]{0.45\textwidth}%
% \textbf{Dialogue} \\
% Dumbledore: And now, Harry, on a closely related subject . . . I gather that you have been taking the Daily Prophet over the last two weeks? \\
% Harry: Yes \\
% ...\\
% % Dumbledore: I think they ought to know. You do them a disservice by not confiding something this important to them. \\
% % Harry: I didn’t want — \\
% Dumbledore: Or perhaps, to confess that you yourself are worried and frightened? You need your friends, Harry. As you so rightly said, Sirius would not have wanted you to shut yourself away.
% \\
% \\
% \textbf{Generated Responses} \\
% GPT: I do not need friends.\\
% Dialog-GPT: He wants to, he wants too much.  \\
% Ori-BOB:  I think they are meaningless...\\
% Per-BOB: It is not your business, because it's my own choice. \\
% \textbf{Expected Response}: Yes, Sirius really doesn't want that, maybe I should talk to them.

% \end{minipage}
% &
% \begin{minipage}[t]{0.45\textwidth}%
% \textbf{Dialogue} \\
% Dudley: Make it move. Do it again...This is boring. \\
% Snake: I get that all the time. \\
% Harry: I know, it mush be really annoying. Where do you come from, anyway? \\
% ...\\
% Pears: DUDLEY! MR. DURSLEY! COME AND LOOK AT THIS SNAKE! YOU WON’T BELIEVE WHAT IT’S DOING! \\
% ... \\
% Pears: Harry was talking to it, weren't you?
% \\
% \\
% \\
% \\
% \\
% \textbf{Generated Responses} \\
% GPT: I do not know... I want to go to Hogwarts.\\
% Dialog-GPT: Sorry, Professor Snape, this is an accident.  \\
% Ori-BOB: I think so, Hagrid.  \\
% Per-BOB: Let us go to see  Hagrid with my owl.\\
% \textbf{Expected Response}: I don't know, you stop talking nonsense, please stop targeting me.
% \end{minipage}
% \\ \bottomrule
% \end{tabular}
% \end{center}
% \vspace{-10pt}
% \caption{Data examples of our dataset and generated responses by baselines (1).}
% \vspace{-10pt}
% \label{table:case_study}
% \end{table*}




\begin{table*}[!t]\footnotesize
% \vspace{-15pt}
\centering
\small
\begin{tabular}{p{1\columnwidth}|p{1\columnwidth}}
% \begin{tabular}{lc}
\toprule
\multicolumn{1}{c}{\textbf{Case-1}} & \multicolumn{1}{c}{\textbf{Case-2}} \\
\midrule
\textbf{Scene} & \textbf{Scene} \\
“And now, Harry, on a closely related subject  . . .  As you so rightly said, Sirius would not have wanted you to shut yourself away.” &   After lunch they went to the reptile house. . . But worst of all, for Harry at least, was Piers calming Belongings enough to say, “Harry was talking to it, weren’t you, Harry?” 	\\
% . . . I gather that you have been taking the Daily Prophet over the last two weeks?”
% “Yes,” said Harry
\midrule
\textbf{Timeline}--Book 6-Chapter 4 & \textbf{Timeline}--Book 1-Chapter 2 \\
% Book 6-Chapter 4  & Book 1-Chapter 2 \\
\textbf{Speakers}--Harry and Dumbledore & \textbf{Speakers}--Harry, Snake, Piers and Dudley\\
 % Harry and Dumbledore & Harry, Snake, Piers and Dudley  \\
\midrule
\textbf{Harry Attributes} & \textbf{Harry Attributes}\\
% Gender: Male & Gender: Male \\
Age: 16 & Age: 11 \\
Talent: Quidditch, Parseltongue & Talent: Parseltongue \\
... & ...
\\
Affiliation: Hogwarts & Affiliation: None \\
% Lineage: None \\
Belongings:  ... Firebolt-Broom, Marauder's Map & Belongings: None	\\
\midrule
	
\textbf{Relations} & \textbf{Relations} \\
Harry's affection for Dumbledore : 6 & Harry's affection for Dudley : -4\\
Harry's familiarity  with Dumbledore : 6 & Harry's familiarity  with Dudley : 6\\
Harry's affection for Sirius : 8 & Harry's affection for Piers : -3\\
Harry's familiarity  with Sirius : 6 & Harry's affection for Piers : 2 \\
... & ... \\
% Harry's familiarity  with Dumbledore : 2\\
	
	 \midrule
\textbf{Dialogue} & \textbf{Dialogue} \\
% {Dumbledore: And now, Harry, on a closely related}  & Dudley: Make it move. Do it again...This is boring.\\
% subject . . . I gather that you have been taking the & Snake: I get that all the time. \\
% ... & Dudley: Make it move. Do it again...This is boring. \\
... & ... \\
Dumbledore:  Although I think you ought to relax it in favor of your friends, Mr. Ronald Weasley and Miss Hermione  & Dudley: Make it move. Do it again...This is boring. Snake: I get that all the time. \\
Granger. Yes,  I think they ought to know. You do them a disservice by not confiding something this important to them. Harry: I didn’t want —&  Harry: I know, it mush be really annoying.  Where do you come from, anyway? Was it nice there? Oh, I see — so you’ve never been to Brazil?\\
% & Harry: I know, it mush be really annoying. Where do you come from, anyway?
 % Harry: I didn’t want —& Dudley: Out of the way, you! \\
Dumbledore: — to worry or frighten them? Or perhaps, to & Snake: Brazil, here I come. . . . Thanksss, amigo.  \\
confess that you yourself are worried and frightened?  & Dudley: Out of the way, you! \\
% Dumbledore: I think they ought to know. You do them a disservice by not confiding something this important to them. \\
% Harry: I didn’t want — \\
 % As you so rightly said, Sirius would not have wanted you to shut yourself away.
{ You need your friends, Harry. As you so rightly said, Sirius would not have wanted you to shut yourself away.}	  & Pears: Harry was talking to it, weren't you? \\
% You need your friends, Harry. As you so rightly said,
	 
	 
% 	 Dudley: Make it move. Do it again...This is boring. \\
% Snake: I get that all the time. \\
% Harry: I know, it mush be really annoying. Where do you come from, anyway? \\
% ...\\
% Pears: DUDLEY! MR. DURSLEY! COME AND LOOK AT THIS SNAKE! YOU WON’T BELIEVE WHAT IT’S DOING! \\
% ... \\
% Pears: Harry was talking to it, weren't you?
\midrule	 
\textbf{Generated Responses} & \textbf{Generated Responses} \\
GPT: I do not need friends. & GPT: I do not know... I want to go to Hogwarts.\\
Dialog-GPT: I know him, he wants me shut myself away. & Dialog-GPT: Sorry, Professor Snape, this is an accident.  \\
Ori-BOB:  I think they are meaningless... & Ori-BOB: I think so, Hagrid.\\
Per-BOB: It is not your business,  it's my own choice. & Per-BOB: Let us go to see  Hagrid with my owl.\\
ChatGPT: Okay, I will tell them about the prophecy. & ChatGPT: I was just asking where it came from.\\
\midrule
\textbf{Expected Response}  & \textbf{Expected Response} \\
\textbf{Harry: Yes, Sirius really doesn't want that, maybe I should talk to them.} & \textbf{Harry: I don't know, you stop talking nonsense, please stop targeting me.} \\
\bottomrule	 
	
% 	GPT: I do not know... I want to go to Hogwarts.\\
% Dialog-GPT: Sorry, Professor Snape, this is an accident.  \\
% Ori-BOB: I think so, Hagrid.  \\
% Per-BOB: Let us go to see  Hagrid with my owl.\\
% \textbf{Expected Response}: I don't know, you stop talking nonsense, please stop targeting me. 
	 
% % \multirow{2}{*}{\textbf{Answer}} & \textbf{Of Course} \\
% % 	& 可以\\
% \multirow{2}{*}{\textbf{Response}} & \textbf{It could affect your Mortgage, but it depends on your income level and assets.} \\
% 	\midrule
% 	\multicolumn{2}{c}{Generated Response-\textit{One stage}} \\
% 	\midrule
% \textbf{GPT} & \\
% \midrule
% \textbf{T5} & \\ 
% \midrule
% \textbf{BART} & It must affect your Mortgage.\\
% + \textbf{Prompt} & It may affect your Mortgage.\\
% \midrule
% \multicolumn{2}{c}{Generated Response-\textit{Two stage}} \\
% \midrule
% \textbf{GPT} & \\
% \midrule
% \textbf{T5} & \\
% \midrule
% \textbf{BART} & Credit loan must affect mortgage \\
% + \textbf{Prompt} & Credit loan could affect mortgage, but depends on assets.\\
% \bottomrule
\end{tabular}
\caption{ Data examples of HPD and generated responses by baselines. Simply, we only present Harry's attributes and discrete relations to other speakers in the example. } \label{table:case_study}
% \vspace{-10pt}
\end{table*}
